Impact of Exchange-Correlation Functionals on Predictions of Phonon Hydrodynamics: A Study of Fluorides, Chlorides, and Hydrides

We employ density functional theory calculations to examine the effect of various exchangecorrelation (XC) functionals, including the Perdew Burke Ernzerhof generalized gradient approximation (PBE), the modified Perdew Burke Ernzerhof generalized gradient approximation (PBEsol), and the local density approximation (LDA), on the electrical, mechanical, and thermal properties of sodium fluoride (NaF), lithium fluoride (LiF), potassium fluoride (KF), sodium chloride (NaCl), potassium chloride (KCl), lithium hydride (LiH), sodium hydride (NaH), and potassium hydride (KH). The lattice thermal conductivity is computed based on an iterative solution of the Boltzmann transport equation (BTE). Based on Guyer's criterion and direct solutions to the linearized BTE, we determine the ballistic, phonon hydrodynamics, and diffusive regimes as a function of length scale and temperature. In addition to confirming previous predictions of phonon hydrodynamics in NaF and LiF, we report novel predictions of phonon hydrodynamics in NaH, LiH, KH, KF, NaCl, and KCl. The impact of isotopes on the calculated lattice thermal conductivity and phonon hydrodynamics windows is also reported. The impact of Meta-GGA and hybrid functionals is also discussed. We find that the selection of a functional impacts the prediction of thermal conductivity and the window for observation of phonon hydrodynamics.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
